Learning Complexity of Simulated Annealing

Simulated annealing is an effective and general means of optimization. It is in fact inspired by metallurgy, where the temperature of a material determines its behavior in thermodynamics. Likewise, in simulated annealing, the actions that the algorithm takes depend entirely on the value of a variable which captures the notion of temperature. Typically, simulated annealing starts with a high temperature, which makes the algorithm pretty unpredictable, and gradually cools the temperature down to become more stable. A key component that plays a crucial role in the performance of simulated annealing is the criteria under which the temperature changes namely, the cooling schedule. Motivated by this, we study the following question in this work: "Given enough samples to the instances of a specific class of optimization problems, can we design optimal (or approximately optimal) cooling schedules that minimize the runtime or maximize the success rate of the algorithm on average when the underlying problem is drawn uniformly at random from the same class?" We provide positive results both in terms of sample complexity and simulation complexity. For sample complexity, we show that $\tilde O(\sqrt{m})$ samples suffice to find an approximately optimal cooling schedule of length $m$. We complement this result by giving a lower bound of $\tilde \Omega(m^{1/3})$ on the sample complexity of any learning algorithm that provides an almost optimal cooling schedule. These results are general and rely on no assumption. For simulation complexity, however, we make additional assumptions to measure the success rate of an algorithm. To this end, we introduce the monotone stationary graph that models the performance of simulated annealing. Based on this model, we present polynomial time algorithms with provable guarantees for the learning problem.

==> figs/abstract.tex <==
This draft contains the ideas concerning the simulated annealing project.

==> figs/ideas.tex <==
\section{Ideas}
Since the number of strategies is exponential, it suffices to draw a polynomial number of instances and find the solution that works best on these instances. Therefore, we need to answer the following question:

\begin{question}
	Given $m \in \mathsf{poly}(n)$ instances of the problem, find a sequence of temperatures that maximizes the average score on these instances.
\end{question}

Let us assume for simplicity that the stationary distribution graph is provided for each instance. Moreover, we call a sequence of temperatures \textit{compatible} with a stationary graph, if one can use that sequence of temperatures to reach the note $t$ in that graph. In this case, we can design a dynamic program to find the smallest sequence of temperatures that is compatible with all $m$ instances in time $O(n^m)$ where $n$ is the size of the stationary graph.

\begin{lemma}\label{lemma:1}
	Let $G_1, G_2, \ldots, G_m$ be $m$ stationary distribution graphs of size $n$. There exists an $O(n^m)$  algorithm that finds the smallest sequence of temperatures that is compatible with all graphs.
\end{lemma}


For the case of monotone stationary graph, we can improve the running time of the algorithm by resorting to approximation logarithms.

\begin{lemma}\label{lemma:2}
	Let $G_1, G_2, \ldots, G_m$ be $m$ monotone stationary distribution graphs of size $n$. There exists a polynomial time algorithm that finds a  sequence of temperatures that is compatible with all graphs. Moreover, the length of the output is at most $O(\log n)$ times more than the optimal solution.
\end{lemma}
\begin{proof}
	We show that the problem reduces to multi-set cover. We assume w.l.o.g. that the vertices of the graphs are numbered from $1$ to $n$ in a way that each node $i$ has an empty edge to node $i-1$. We say an edge $e$ covers a vertex $i$ if the starting node of $e$ is before node $i$ and the ending node of $e$ is \textbf{not} before node $i$. Since the graphs are monotone, we need to include a set of edges in our solution such that all vertices (except the source nodes) of all graphs are covered. This reduces the problem to multi-set cover and thus it can be approximated within a factor $O(\log n)$ in polynomial time.
	
	\input{figs/dag3}
	
\end{proof}
 



==> figs/model.tex <==
\section{Model}
Of course, the simplest way to model the problem is via a single temperature which makes the problem somewhat trivial . In general, it can be shown that one can discretize the space of temperatures by imposing a small additive error to the accuracy of the solution. This leaves us with a set of (polynomially many) temperatures that we denote by $\infty > t_1 > t_2 > t_3 > \ldots > t_{\tsize}$ (\color{red}\textsf{needs explanation}\color{black}). Thus, w.l.o.g we focus our attention on the discretized setting.

To go beyond the single temperature setting, we define a schedule to be a non-increasing sequence of temperatures $\para = \langle t_{a_1}, t_{a_2}, \ldots, t_{a_m}\rangle$ where each $t_{a_i}$ denote the temperature at time step $i$. Based on the parameters of $\para$, our \textsf{SA} algorithm makes an uphill move at time $i$ with probability 
$$\mathsf{Pr}[\text{ accepting an uphill move at time step }i] \simeq 1 - e^{\Delta(E)/ t_{a_i}}.$$

If after $m$ steps our \textsf{SA} algorithms finds a solution, then we give a score $1$ to $\para$ and otherwise we give a score $0$ to $\para$. Thus, $\score$ is defined as the probability of finding a correct solution after $m$ steps.

One can observe that even after discretizing the space of temperatures, we have an exponentially large set of options for $\para$ and therefore computing the right sequence of temperatures even for a fixed instance $\mathsf{I}$ of the problem is not trivial. The sampling complexity however is not so challenging as it usually depends logarithmically on the space of parameters (\color{red}\textsf{needs explanation}\color{black}).

Here we bring some (hopefully defensible) assumptions that may help us obtain a nontrivial solution:
\begin{itemize}
	\item (\textit{monotonicity}). Let $\para_1$ be a sequence of temperatures for $m_1$ steps of \textsf{SA} and $\para_2$ be a sequence of temperatures for $m_2 \geq m_1$ steps of \textsf{SA}. If $\para_1$ is a subsequence of $\para_2$, then running $m_2$ steps of \textsf{SA} on $\para_2$ is always at least as good as running \textsf{SA} on $m_1$ steps of $\para_1$ (in expectation).
	
	\item (\textit{stationary distribution graph}). For a fixed instance $\mathsf{I}$ of the problem, define a stationary distribution graph $\graph(\mathsf{I})$ that describes the state of a random walk or \textsf{SA}. Therefore, after performing \textsf{SA} on a sequence of temperatures, the distribution of nodes that the algorithm will be at is described by a node of $\graph(\mathsf{I})$. More precisely, each node of graph $\mathsf{I}$, corresponds to a single temperature $t_i$. Thus, if we manage to reach node $t_i$ using a sequence of temperatures, it means that we are currently at the stationary distribution for $t_i$. Therefore, we abuse tho notation and also refer to each node of graph $\mathsf{I}$ by $t_i$ for some integer $0 \leq i \leq \tsize$. Node $t_0$ is a special node which does not correspond to any temperature, however, our algorithm initially starts at node $t_0$.
		
	 Transitions between the stationary distributions are shown via edges in $\graph(\mathsf{I})$. Each edge is associated with a sequence of temperatures that make the transition possible from a specific node $x$ to a specific node $y$. For instance, an edge from state $t_2$ to state $t_5$ with label $t_5, t_5, t_5$ means that for any sequence $\para$ of temperatures that  brings us to state $t_2$, $\para . [t_5, t_5, t_5]$\footnote{$.$ here stands for concatenation.} takes us to state $t_5$. Thus, if for a given instance $\mathsf{I}$ the stationary graph is provided, one can find the optimal sequence of temperatures via a shortest path algorithm. Also, all the edges that point to a node $t_i$ only contain temperature $t_i$. However, each edge require a different number of $t_i$ temperatures to take us to node $t_i$.  
	
	\input{figs/dag1}
	
	\input{figs/dag2}
	
\end{itemize}

==> figs/model_2.tex <==
\section{Model}
Of course, the simplest way to model the problem is via a single temperature which makes the problem somewhat trivial . In general, it can be shown that one can discretize the space of temperatures by imposing a small additive error to the accuracy of the solution. This leaves us with a set of (polynomially many) temperatures that we denote by $\infty > t_1 > t_2 > t_3 > \ldots > t_{\tsize}$ (\color{red}\textsf{needs explanation}\color{black}). Thus, w.l.o.g we focus our attention on the discretized setting.

To go beyond the single temperature setting, we define a schedule to be a non-increasing sequence of temperatures $\para = \langle t_{a_1}, t_{a_2}, \ldots, t_{a_m}\rangle$ where each $t_{a_i}$ denote the temperature at time step $i$. Based on the parameters of $\para$, our \textsf{SA} algorithm makes an uphill move at time $i$ with probability 
$$\mathsf{Pr}[\text{ accepting an uphill move at time step }i] \simeq 1 - e^{\Delta(E)/ t_{a_i}}.$$

If after $m$ steps our \textsf{SA} algorithms finds a solution, then we give a score $1$ to $\para$ and otherwise we give a score $0$ to $\para$. Thus, $\score$ is defined as the probability of finding a correct solution after $m$ steps.

One can observe that even after discretizing the space of temperatures, we have an exponentially large set of options for $\para$ and therefore computing the right sequence of temperatures even for a fixed instance $\mathsf{I}$ of the problem is not trivial. The sampling complexity however is not so challenging as it usually depends logarithmically on the space of parameters (\color{red}\textsf{needs explanation}\color{black}).

Here we bring some (hopefully defensible) assumptions that may help us obtain a nontrivial solution:
\begin{itemize}
	\item (\textit{monotonicity}). Let $\para_1$ be a sequence of temperatures for $m_1$ steps of \textsf{SA} and $\para_2$ be a sequence of temperatures for $m_2 \geq m_1$ steps of \textsf{SA}. If $\para_1$ is a subsequence of $\para_2$, then running $m_2$ steps of \textsf{SA} on $\para_2$ is always at least as good as running \textsf{SA} on $m_1$ steps of $\para_1$ (in expectation).
	
	\item (\textit{stationary distribution graph}). For a fixed instance $\mathsf{I}$ of the problem, define a stationary distribution graph $\graph(\mathsf{I})$ that describes the state of a random walk or \textsf{SA}. Therefore, after performing \textsf{SA} on a sequence of temperatures, the distribution of nodes that the algorithm will be at is described by a node of $\graph(\mathsf{I})$. More precisely, each node of graph $\mathsf{I}$, corresponds to a single temperature $t_i$. Thus, if we manage to reach node $t_i$ using a sequence of temperatures, it means that we are currently at the stationary distribution for $t_i$. Therefore, we abuse tho notation and also refer to each node of graph $\mathsf{I}$ by $t_i$ for some integer $0 \leq i \leq \tsize$. Node $t_0$ is a special node which does not correspond to any temperature, however, our algorithm initially starts at node $t_0$.
		
	 Transitions between the stationary distributions are shown via edges in $\graph(\mathsf{I})$. Each edge is associated with a sequence of temperatures that make the transition possible from a specific node $x$ to a specific node $y$. For instance, an edge from state $t_2$ to state $t_5$ with label $t_5, t_5, t_5$ means that for any sequence $\para$ of temperatures that  brings us to state $t_2$, $\para . [t_5, t_5, t_5]$\footnote{$.$ here stands for concatenation.} takes us to state $t_5$. Thus, if for a given instance $\mathsf{I}$ the stationary graph is provided, one can find the optimal sequence of temperatures via a shortest path algorithm. Also, all the edges that point to a node $t_i$ only contain temperature $t_i$. However, each edge require a different number of $t_i$ temperatures to take us to node $t_i$.  
	
	\input{figs/dag1}
	
	\input{figs/dag2}
	
\end{itemize}

==> src/dag-bad.tex <==
\begin{figure}[H]\centering
	\begin{tikzpicture}[node distance=1.3cm,>=stealth',bend angle=45,auto]
	
	\tikzstyle{place}=[circle,thick,draw=blue!75,fill=blue!20,minimum size=6mm]
	\tikzstyle{red place}=[place,draw=red!75,fill=red!20]
	\tikzstyle{transition}=[rectangle,thick,draw=black!75,
	fill=red,minimum size=4mm]
	
	\tikzstyle{every label}=[red]
	
	\begin{scope}
	  [align=center,node distance=3cm]  %< no need of this global node separation
	
	% First net
	\node [transition] (w1) {$t_0$};
	\node [place] (w2) [right of=w1] {$t_1$} edge [pre,color=magenta] node[swap] {$\langle t_1, t_1, t_1\rangle$} (w1) ;
	\node [place] (w3) [right of=w2] {$t_2$} edge [pre] node[swap] {$\langle t_2, t_2\rangle$} (w2) edge [pre,bend right,color=blue] node[swap] {$\langle t_2, t_2, t_2, t_2\rangle$} (w1) ;
	\node [place] (w4) [right of=w3] {$t_3$}  edge [pre, bend left] node[swap] {$\langle t_3, t_3, t_3, t_3\rangle$} (w2) edge [pre] node[swap] {$\langle t_3, t_3\rangle$} (w3);
	\node [place] (w5) [right of=w4] {$t_4$} edge [pre] node[swap] {$\langle t_4, t_4, t_4\rangle$} (w4) ;
	\node [place] (w6) [right of=w5] {$t_5$} edge [pre] node[swap] {$\langle t_5, t_5\rangle$} (w5) {} edge [pre, bend right,color=magenta] node[swap] {$\langle t_5, t_5, t_5,t_5, t_5, t_5\rangle$} (w2);
  \end{scope}
	
	
	\end{tikzpicture}
	\caption{A sequence $\langle \color{blue}t_1, t_1, t_1,\color{red} t_5, t_5, t_5, t_5, t_5, t_5\color{black}\rangle$ takes us to node $t_5$. However, a sequence $\langle \color{blue}t_2, t_2, t_2, t_2,\color{red} t_5, t_5, t_5, t_5, t_5, t_5\color{black}\rangle$ takes us to node $t_2$.}\label{fig:dagbad}
\end{figure}

==> src/empirical.tex <==
\section{Empirical Results}\label{sec:empirical}


==> src/model.tex <==
\subsection{Monotone Stationary Graphs}\label{sec:monotone}
Our model is based on a stationary graph and adheres to a certain structure which also guarantees monotonicity. To this end, fix an instance $\mathsf{I}$ of the problem and denote its stationary graph by $\graph(\mathsf{I})$. Recall that the states of the stationary graph correspond to the temperatures (except the initial node which we denote by $v_0$). Our assumption in this case is that the success probability of the algorithm for a sequence $\para$ depends on the node that $\para$ takes us to in $\graph(\mathsf{I})$. Indeed, we expect probability to increase as we reach the stationary distributions for low temperatures. Thus, we define a score $s_i$ for every node $v_i$ of $\graph(\mathsf{I})$ and assume that $s_0 \leq s_1 \leq s_2 \leq \ldots \leq s_{\tsize} \leq 1$ holds for the scores. Roughly speaking, $s_i$ reflects the success probability of a sequence of temperatures $\para$ that takes us to the stationary distribution of $t^i$ in $\graph(\mathsf{I})$. 


One problem that raises here is that in this model, nodes with lower temperatures are not necessarily better that nodes with higher temperatures even though they have higher scores. Let us highlight this point with an example.
In Figure \ref{fig:dagbad}, we have a stationary graph with nodes $v_0$ through $v_5$. In this example, a sequence $\langle t^1, t^1, t^1 \rangle$  takes us to node $v_1$ and then using a sequence $\langle t^5, t^5, t^5, t^5, t^5, t^5\rangle$ we can reach node $v_5$. Thus, the combination of the two sequences ($\langle \color{blue}t^1, t^1, t^1,\color{red} t^5, t^5, t^5, t^5, t^5, t^5\color{black}\rangle$) takes us to node $v_5$. However, assume that instead of sequence  $\langle t^1, t^1, t^1 \rangle$ we start with $\langle t^2, t^2, t^2, t^2\rangle$ which is supposed to take us to a \textit{better} node. In this case, after combining $\langle t^5, t^5, t^5, t^5, t^5, t^5 \rangle$ with $\langle t^2, t^2, t^2, t^2\rangle$ we still stay at $v_2$. This is counter-intuitive since combining $\langle t^5, t^5, t^5, t^5, t^5, t^5 \rangle$  with $\langle t^1, t^1, t^1\rangle$ takes us to node $v_5$.

\input{figs/dag-bad}

In addition to the above, it is not clear what happens if we perform a step multiple times. For instance, does $\langle \color{blue}t^1, t^1, t^1, t^1,\color{red} t^5, t^5, t^5, t^5, t^5, t^5\color{black}\rangle$ still take us to node $v_5$ or the addition of the extra $t^1$ breaks the solution? We resolve these two issues by manually enforcing monotonicity to the model. To resolve the former problem, we add an edge from every node $v_i$ to its previous node $v_{i-1}$ with an empty label. This means that any sequence of temperatures that takes us to a node $v_i$ can also take us to a node $v_{j}$ for any $j < i$. To address the second issue, we add an edge from every node $v_i$ to itself with a label $t^i$. This means that if you make several steps of a single temperature, the solution does not hurt. The combination of these to modifications provides monotonicity in the following senses:
\begin{itemize}
	\item For every instance $\mathsf{I}$ of the problem and any two sequences $\para_1$ and $\para_2$ of the temperatures such that $\para_1$ is as subsequence of $\para_2$ we have $\score(\mathsf{I},\para_1) \leq  \score(\mathsf{I},\para_2)$. 
	\item Any sequence of temperatures that takes us to a node $v_i$ is always no worse than a sequence of temperatures that has no path to node $v_i$ (\color{red}\textsf{If the sequence is taking you further in the graph, then your algorithm is doing better}\color{black}). 
\end{itemize}

The application of the above two ideas to the example of Figure \ref{fig:dagbad} gives us the graph in Figure \ref{fig:daggood}. In Section \ref{sec:learning}, we discuss how one can learn the monotone stationary graph.

\input{figs/dag2}

%\color{red}\textsf{downside of this model: }\color{black} We acknowledge that this model suffers from the following counter-intuitive phenomenon. Suppose there is an edge from vertex $t^i$ to vertex $t^j$ whose label is $\overbrace{\langle t^j, t^j, \ldots, t^j\rangle}^{100}$. If we append 99 $t^j$'s to a sequence that already takes us to node $t^i$, we still remain at node $t^i$ although we have traversed $99\%$ of the last edge. This is hard to justify since the transition between the stations is made gradually in practice. \color{red}\textsf{this seems to be one sacrifice we have to make in order to make the problem tractable.}\color{black}


==> tables/notation.tex <==
\begin{table}[!htbp]
	\centering
	\begin{tabular}{|l|l|}
		\hline
		\rowcolor{LightCyan}notation & meaning\\
		\hline
		$m$ &the size of the optimal solution\\
		\hline
		$n$ &the number of samples used to learn a cooling schedule\\
		\hline
		$t_i$ & $i$'th temperature used is a cooling schedule\\
		\hline
		$d_{i}$ & $i$'th temperature in the discretized set\\
		\hline 
		$\para = \{t_1, t_2,\ldots,t_m\}$ & a cooling schedule\\
		\hline
		$T = \{d_{1}, d_{2},\ldots,d_{|T|}\}$ & the set of discretized temperatures\\
		\hline
		$\score(\para,\ii)$& the score of a cooling schedule $\para$ on an instance $\ii$ of the problem\\ 
		\hline
		$\distribution$ & A distribution of instances corresponding to the class of pertinent problem\\
		\hline
	\end{tabular}
\caption{Our notations are summarized in this table.}
\end{table}\label{table:notation}


